Portability of Fortran's `do concurrent' on GPUs

There is a continuing interest in using standard language constructs for accelerated computing in order to avoid (sometimes vendor-specific) external APIs. For Fortran codes, the {\tt do concurrent} (DC) loop has been successfully demonstrated on the NVIDIA platform. However, support for DC on other platforms has taken longer to implement. Recently, Intel has added DC GPU offload support to its compiler, as has HPE for AMD GPUs. In this paper, we explore the current portability of using DC across GPU vendors using the in-production solar surface flux evolution code, HipFT. We discuss implementation and compilation details, including when/where using directive APIs for data movement is needed/desired compared to using a unified memory system. The performance achieved on both data center and consumer platforms is shown.

==> AD.tex <==

Artifact Identification:

(i) an abstract describing the main contributions of the article and the role of the computational artifact(s) in these contributions.

(ii) the abstract may include a software architecture or data models and its description to help the readers understand the computational artifact(s)

(iii) a clear description on to what extent the computational artifact(s) contribute(s) to the reproducibility of the experiments in the article.

%START_LATEX
We have investigated the portability of using Fortran's `do concurrent` (DC) for accelerated computing by testing its use across GPU vendors using the solar flux evolution code HipFT.  HipFT is written using DC loops and includes OpenMP target data directives for manual data movement between the CPU and GPU for platforms that do not support (or have non-optimal) automatic data management.  We successfully compiled and ran a production-level test case on NVIDIA, Intel, and AMD GPUs using NVIDIA's HPC SDK's {\tt nvfortran}, Intel's OneAPI HPC Toolkit's {\tt ifx}, and HPE's Cray Compiler Environment's {\tt ftn} compilers respectively. Both server and consumer hardware were tested.  Tags/releases of the github repository of HipFT (\url{https://github.com/predsci/hipft}) were made for the versions used in this paper, specifically the {\tt v1.11.0} release of the code was used for CPU runs and the NVIDIA GPU and AMD GPU runs. The {\tt v1.11.0-intel-gpu} branch release (only 6 modified lines) was used for Intel GPU runs.    The test case is the run located in the {\tt examples/flux\_transport\_1rot\_flowAa\_diff\_r8} folder of the HipFT github repository.  Given access to the computational hardware, the repository with its release tags can be used to directly reproduce the run timings shown in the paper by building with the compiler flags described in the paper, along with any/all system-specific compiler flags that may be needed.  The HipFT code outputs a breakdown of the time taken in each section of the code, and this data is used to generate the bar plots in the figures.
%STOP_LATEX


Reproducibility of Experiments

i) a complete description of the experiment workflow that the computational artifact(s) can execute

(ii) an estimation of the execution time to execute the experiment workflow.

(iii) a complete description of the expected results and an evaluation of them, and most importantly.

(iv) how the expected results from the experiment workflow relate to the results found in the article. 

%START_LATEX
The workflow to generate the results in this paper is as follows:  First, checkout the relevant release of HipFT (either \url{github.com/predsci/HipFT/releases/tag/v1.11.0} for NVIDIA and AMD GPUs or \url{github.com/predsci/HipFT/releases/tag/v1.11.0-intel-gpu} for Intel GPUs.  Next, build the code according to the build instructions (including having an HDF5 library installed with the same compiler used for HipFT), the included sample build scripts, and the compiler flags described in the paper.  Then, copy the input files from the {\tt examples/flux\_transport\_1rot\_flowAa\_diff\_r8} folder into a new folder, and run the code with {\tt mpirun -np <N> hipft} (assuming HipFT is in your run path) and where {\tt <N>} is the number of MPI ranks to use (in this case, typically 1).

The execution time will depend on the hardware and software platforms.  If running on similar hardware as described in the paper, the run times should be very close to  those in the bar plots (maximum $\sim1$hr), except possibly for the gray "other" area which can be sensitive to the speed of the file system.

If the test case is run on the same hardware and software versions (including compilers) are done in the paper, it is expected to get very similar run times as those shown in the bar plots.  The results should show the portability of Fortran's DC for GPU acceleration, with similar timings for NVIDIA and Intel GPUs of comparable capabilities, as well as correct execution on AMD GPUs.   Running the tests with newer versions of the compilers, or on newer GPU hardware should result in faster run times.
%STOP_LATEX
